ML Codebook Design for Initial Access and CSI Type-II Feedback in Sub-6GHz 5G NR

Beam codebooks are a recent feature to enable high dimension multiple-input multiple-output in 5G. Codebooks comprised of customizable beamforming weights can be used to transmit reference signals and aid the channel state information (CSI) acquisition process. Codebooks are also used for quantizing feedback following CSI acquisition. In this paper, we characterize the role of each codebook used during the beam management process and design a neural network to find codebooks that improve overall system performance. Evaluating a codebook requires considering the system-level dependency between the codebooks, feedback, overhead, and spectral efficiency. The proposed neural network is built on translating codebook and feedback knowledge into a consistent beamspace basis similar to a virtual channel model to generate initial access codebooks. This beamspace codebook algorithm is designed to directly integrate with current 5G beam management standards without changing the feedback format or requiring additional side information. Our simulations show that the neural network codebooks improve over traditional codebooks, even in dispersive sub-6GHz environments. We further use our framework to evaluate CSI feedback formats with regard to multi-user spectral efficiency. Our results suggest that optimizing codebook performance can provide valuable performance improvements, but optimizing the feedback configuration is also important in sub-6GHz bands.

==> IEEEabrv.tex <==
%%
%% IEEEabrv.bib
%%
%% BibTeX bibliography string definitions of the ABBREVIATED titles of
%% IEEE journals and magazines
%% 
%% NOTE: This text file uses MS Windows line feed conventions. When (human)
%% reading this file on other platforms, you may have to use a text
%% editor that can handle lines terminated by the MS Windows line feed
%% characters (0x0D 0x0A).
%%
%% This file is designed for bibliography styles that require 
%% abbreviated titles and is not for use in bibliographies that
%% require full-length titles.
%% 
%% Version 1.10 (2003/04/02)
%% 
%% Composed by Michael Shell
%% 
%% See:
%% http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/
%% for latest version and current contact information.
%%
%% Special thanks to Laura Hyslop of IEEE for her help in obtaining the
%% information needed to compile this file. Also, Volker Kuhlmann kindly
%% provided some corrections and additions.
%%
%%**********************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE!
%% User assumes all risk.
%% In no event shall IEEE or any contributor to this code be liable for
%% any damages or losses, including, but not limited to, incidental,
%% consequential, or any other damages, resulting from the use or misuse
%% of any information contained here.
%%
%% This code is distributed under the Perl Artistic License 
%% ( http://language.perl.com/misc/Artistic.html ) 
%% and may be freely used, distributed and modified - subject to the
%% constraints therein.
%% Retain all contribution notices, credits and disclaimers.
%% 
%% All comments are the opinions of their respective authors and are not
%% necessarily endorsed by the IEEE.
%%**********************************************************************
%
%
% USAGE:
% 
% \bibliographystyle{mybstfile} 
% \bibliography{IEEEabrv,mybibfile}
%
% where the IEEE titles in the .bib database entries use the strings
% defined here. e.g.,
%
%
%    journal = IEEE_J_AC,
%
%
% to yield "{IEEE} Trans. Automat. Contr."
%
%
% IEEE uses abbreviated journal titles in their bibliographies -
% this file is suitable for work that is to be submitted to the IEEE.
%
%
% For work that requires full-length titles, you should use the full
% titles provided in the companion file, IEEEfull.bib.
%
%
% ** NOTES **
%
% 1. Journals have been grouped according to subject in order to make it
%    easier to locate and extract the definitions for related journals - 
%    as most works use references that are confined to a single topic.
%    Magazines are listed in straight alphabetical order.
%
% 2. String names are closely based on IEEE's own internal acronyms.
% 
% 3. Abbreviations follow IEEE's style.
%
% 4. Older, out-of-print IEEE titles are included (but not including titles
%    dating prior to IEEE's formation from the IRE and AIEE in 1963).
%
% 5. The following NEW/current journal definitions have been disabled because
%    their abbreviations have not yet been finalized/verified:
%    
%    STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
%    STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
%    STRING{IEEE_J_MCTE       = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
%    STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochemical Solid-State Lett."}
%    STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
%    
% 6. The following OLD journal definitions have been disabled because
%    their abbreviations have not yet been found/verified:
%
%    STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
%    STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
%
% If you know what the proper abbreviation is for a string in #5 or #6 above,
% email me and I will correct them in the next release.

%%%%%%%%%%%%%%%%%%%
%% Dates %%
%%%%%%%%%%%%%%%%%%%
@STRING{jan. = "Jan."}
@STRING{feb. = "Feb."}
@STRING{march = "March"}
@STRING{april = "April"}
@STRING{may = "May"}
@STRING{june = "June"}
@STRING{july = "July"}
@STRING{aug. = "Aug."}
@STRING{sep. = "Sep."}
@STRING{oct. = "Oct."}
@STRING{nov. = "Nov."}
@STRING{dec. = "Dec."}




%%%%%%%%%%%%%%%%%%%
%% IEEE Journals %%
%%%%%%%%%%%%%%%%%%%


% aerospace and military
@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



% autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transport. Syst."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}



% circuits, signals, systems, audio and controls
@STRING{IEEE_J_SPL        = "{IEEE} Signal Processing Lett."}
@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Processing"}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Automat. Contr."}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Trans. Contr. Syst. Technol."}
@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Processing"}
@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Processing"}
@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelect., Freq. Contr."}
@STRING{IEEE_J_JSTSP       = "{IEEE} J. Select. Topics Signal Processing"}



% communications
@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Select. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}



% components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Comp., Hybrids, Manufact. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {B}"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {C}"}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CPART      = "{IEEE} Trans. Comp. Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manufact."}
@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manufact. Technol."}
@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



% CAD
@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Computer Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Trans. Computer-Aided Design"}



% coding, data, information, knowledge
@STRING{IEEE_J_IT         = "{IEEE} Trans. Inform. Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowledge Data Eng."}



% computers, computation, networking and software
@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
% disabled till definition finalized
STRING{IEEE_J_MC          = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Networking"}
@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Networks"}
@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SE         = "{IEEE} Trans. Software Eng."}



% computer graphics, imaging, and multimedia
@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Processing"}
@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Trans. Visual. Comput. Graphics"}



% cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Automat."}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Machine Intell."}
@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Automat."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybernetics"}



% earth, wind, fire and water
@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sensing"}
@STRING{IEEE_J_OE         = "{IEEE} J. Oceanic Eng."}



% education, engineering, history, IEEE, professional
% disabled till definition is verified
STRING{IEEE_J_CJECE       = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manage."}
% disabled till definition is verified
STRING{IEEE_J_EWS         = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



% electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propagat. Lett."}
@STRING{IEEE_J_MGWL       = "{IEEE} Microwave Guided Wave Lett."}
% IEEE seems to want "Compon." here, not "Comp."
@STRING{IEEE_J_MWCL       = "{IEEE} Microwave Wireless Compon. Lett."}
@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propagat."}
@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microwave Theory Tech."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



% energy and power
@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Conversion"}
@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Delivery"}
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}



% industrial, commercial and consumer
@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Applicat. Ind."}
@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
% disabled till definition is verified
STRING{IEEE_J_BCTV        = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Trans. Consumer Electron."}
@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Applicat."}
@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Applicat."}



% instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



% insulation and materials
% disabled till definition finalized
STRING{IEEE_J_JEM         = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielect. Elect. Insulation"}
@STRING{IEEE_J_EI         = "{IEEE} Trans. Elect. Insulation"}



% mechanical
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatron."}
@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}



% medical and biological
@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
% Note: The B-ME journal later dropped the hyphen and became the BME.
@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inform. Technol. Biomed."}
@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
% disabled till definition finalized
STRING{IEEE_J_MCTE        = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehab. Eng."}
@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehab. Eng."}



% optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_JLT        = "J. Lightwave Technol."}



% physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Select. Topics Quantum Electron."}
@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



% reliability
% IEEE seems to want "Mat." here, not "Mater."
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mat. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



% semiconductors, superconductors, electrochemical and solid state
% disabled till definition finalized
STRING{IEEE_J_ESSL        = "{IEEE/ECS} Electrochemical Solid-State Lett."}
@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Superconduct."}
@STRING{IEEE_J_SM         = "{IEEE} Trans. Semiconduct. Manufact."}



% sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



% VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}





%%%%%%%%%%%%%%%%%%%%
%% IEEE Magazines %%
%%%%%%%%%%%%%%%%%%%%


@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag"}
@STRING{IEEE_M_HIST       = "{IEEE} Annals Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propagat. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
% CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microwave"}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NET        = "{IEEE} Network"}
% IEEE's editorial manual lists "Pers. Commun.", 
% but "Personal Commun. Mag." seems to be what is used in the journals
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
% CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Automat. Mag."}
@STRING{IEEE_M_SP         = "{IEEE} Signal Processing Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun. Mag."}
@STRING{IEEE_M_TODAY      = "Today's Eng."}




%--
%EOF


==> Initial Access Codebook Design and CSI Type-II Feedback for Sub-6GHz 5G NR/IEEEabrv.tex <==
%%
%% IEEEabrv.bib
%%
%% BibTeX bibliography string definitions of the ABBREVIATED titles of
%% IEEE journals and magazines
%% 
%% NOTE: This text file uses MS Windows line feed conventions. When (human)
%% reading this file on other platforms, you may have to use a text
%% editor that can handle lines terminated by the MS Windows line feed
%% characters (0x0D 0x0A).
%%
%% This file is designed for bibliography styles that require 
%% abbreviated titles and is not for use in bibliographies that
%% require full-length titles.
%% 
%% Version 1.10 (2003/04/02)
%% 
%% Composed by Michael Shell
%% 
%% See:
%% http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/
%% for latest version and current contact information.
%%
%% Special thanks to Laura Hyslop of IEEE for her help in obtaining the
%% information needed to compile this file. Also, Volker Kuhlmann kindly
%% provided some corrections and additions.
%%
%%**********************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE!
%% User assumes all risk.
%% In no event shall IEEE or any contributor to this code be liable for
%% any damages or losses, including, but not limited to, incidental,
%% consequential, or any other damages, resulting from the use or misuse
%% of any information contained here.
%%
%% This code is distributed under the Perl Artistic License 
%% ( http://language.perl.com/misc/Artistic.html ) 
%% and may be freely used, distributed and modified - subject to the
%% constraints therein.
%% Retain all contribution notices, credits and disclaimers.
%% 
%% All comments are the opinions of their respective authors and are not
%% necessarily endorsed by the IEEE.
%%**********************************************************************
%
%
% USAGE:
% 
% \bibliographystyle{mybstfile} 
% \bibliography{IEEEabrv,mybibfile}
%
% where the IEEE titles in the .bib database entries use the strings
% defined here. e.g.,
%
%
%    journal = IEEE_J_AC,
%
%
% to yield "{IEEE} Trans. Automat. Contr."
%
%
% IEEE uses abbreviated journal titles in their bibliographies -
% this file is suitable for work that is to be submitted to the IEEE.
%
%
% For work that requires full-length titles, you should use the full
% titles provided in the companion file, IEEEfull.bib.
%
%
% ** NOTES **
%
% 1. Journals have been grouped according to subject in order to make it
%    easier to locate and extract the definitions for related journals - 
%    as most works use references that are confined to a single topic.
%    Magazines are listed in straight alphabetical order.
%
% 2. String names are closely based on IEEE's own internal acronyms.
% 
% 3. Abbreviations follow IEEE's style.
%
% 4. Older, out-of-print IEEE titles are included (but not including titles
%    dating prior to IEEE's formation from the IRE and AIEE in 1963).
%
% 5. The following NEW/current journal definitions have been disabled because
%    their abbreviations have not yet been finalized/verified:
%    
%    STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
%    STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
%    STRING{IEEE_J_MCTE       = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
%    STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochemical Solid-State Lett."}
%    STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
%    
% 6. The following OLD journal definitions have been disabled because
%    their abbreviations have not yet been found/verified:
%
%    STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
%    STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
%
% If you know what the proper abbreviation is for a string in #5 or #6 above,
% email me and I will correct them in the next release.

%%%%%%%%%%%%%%%%%%%
%% Dates %%
%%%%%%%%%%%%%%%%%%%
@STRING{jan. = "Jan."}
@STRING{feb. = "Feb."}
@STRING{march = "March"}
@STRING{april = "April"}
@STRING{may = "May"}
@STRING{june = "June"}
@STRING{july = "July"}
@STRING{aug. = "Aug."}
@STRING{sep. = "Sep."}
@STRING{oct. = "Oct."}
@STRING{nov. = "Nov."}
@STRING{dec. = "Dec."}




%%%%%%%%%%%%%%%%%%%
%% IEEE Journals %%
%%%%%%%%%%%%%%%%%%%


% aerospace and military
@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



% autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transport. Syst."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}



% circuits, signals, systems, audio and controls
@STRING{IEEE_J_SPL        = "{IEEE} Signal Processing Lett."}
@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Processing"}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Automat. Contr."}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Trans. Contr. Syst. Technol."}
@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Processing"}
@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Processing"}
@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelect., Freq. Contr."}
@STRING{IEEE_J_JSTSP       = "{IEEE} J. Select. Topics Signal Processing"}



% communications
@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Select. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}



% components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Comp., Hybrids, Manufact. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {B}"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {C}"}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CPART      = "{IEEE} Trans. Comp. Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manufact."}
@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manufact. Technol."}
@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



% CAD
@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Computer Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Trans. Computer-Aided Design"}



% coding, data, information, knowledge
@STRING{IEEE_J_IT         = "{IEEE} Trans. Inform. Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowledge Data Eng."}



% computers, computation, networking and software
@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
% disabled till definition finalized
STRING{IEEE_J_MC          = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Networking"}
@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Networks"}
@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SE         = "{IEEE} Trans. Software Eng."}



% computer graphics, imaging, and multimedia
@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Processing"}
@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Trans. Visual. Comput. Graphics"}



% cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Automat."}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Machine Intell."}
@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Automat."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybernetics"}



% earth, wind, fire and water
@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sensing"}
@STRING{IEEE_J_OE         = "{IEEE} J. Oceanic Eng."}



% education, engineering, history, IEEE, professional
% disabled till definition is verified
STRING{IEEE_J_CJECE       = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manage."}
% disabled till definition is verified
STRING{IEEE_J_EWS         = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



% electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propagat. Lett."}
@STRING{IEEE_J_MGWL       = "{IEEE} Microwave Guided Wave Lett."}
% IEEE seems to want "Compon." here, not "Comp."
@STRING{IEEE_J_MWCL       = "{IEEE} Microwave Wireless Compon. Lett."}
@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propagat."}
@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microwave Theory Tech."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



% energy and power
@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Conversion"}
@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Delivery"}
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}



% industrial, commercial and consumer
@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Applicat. Ind."}
@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
% disabled till definition is verified
STRING{IEEE_J_BCTV        = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Trans. Consumer Electron."}
@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Applicat."}
@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Applicat."}



% instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



% insulation and materials
% disabled till definition finalized
STRING{IEEE_J_JEM         = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielect. Elect. Insulation"}
@STRING{IEEE_J_EI         = "{IEEE} Trans. Elect. Insulation"}



% mechanical
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatron."}
@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}



% medical and biological
@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
% Note: The B-ME journal later dropped the hyphen and became the BME.
@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inform. Technol. Biomed."}
@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
% disabled till definition finalized
STRING{IEEE_J_MCTE        = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehab. Eng."}
@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehab. Eng."}



% optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_JLT        = "J. Lightwave Technol."}



% physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Select. Topics Quantum Electron."}
@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



% reliability
% IEEE seems to want "Mat." here, not "Mater."
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mat. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



% semiconductors, superconductors, electrochemical and solid state
% disabled till definition finalized
STRING{IEEE_J_ESSL        = "{IEEE/ECS} Electrochemical Solid-State Lett."}
@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Superconduct."}
@STRING{IEEE_J_SM         = "{IEEE} Trans. Semiconduct. Manufact."}



% sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



% VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}





%%%%%%%%%%%%%%%%%%%%
%% IEEE Magazines %%
%%%%%%%%%%%%%%%%%%%%


@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag"}
@STRING{IEEE_M_HIST       = "{IEEE} Annals Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propagat. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
% CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microwave"}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NET        = "{IEEE} Network"}
% IEEE's editorial manual lists "Pers. Commun.", 
% but "Personal Commun. Mag." seems to be what is used in the journals
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
% CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Automat. Mag."}
@STRING{IEEE_M_SP         = "{IEEE} Signal Processing Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun. Mag."}
@STRING{IEEE_M_TODAY      = "Today's Eng."}




%--
%EOF

